Fast and Memory-Efficient Significant Pattern Mining via Permutation Testing

We present a novel algorithm, Westfall-Young light, for detecting patterns, such as itemsets and subgraphs, which are statistically significantly enriched in one of two classes. Our method corrects rigorously for multiple hypothesis testing and correlations between patterns through the Westfall-Young permutation procedure, which empirically estimates the null distribution of pattern frequencies in each class via permutations. In our experiments, Westfall-Young light dramatically outperforms the current state-of-the-art approach in terms of both runtime and memory efficiency on popular real-world benchmark datasets for pattern mining. The key to this efficiency is that unlike all existing methods, our algorithm neither needs to solve the underlying frequent itemset mining problem anew for each permutation nor needs to store the occurrence list of all frequent patterns. Westfall-Young light opens the door to significant pattern mining on large datasets that previously led to prohibitive runtime or memory costs.

==> background.tex <==
\section{Background}
\label{sec:background}

{\bf M: I think we should do numbering subsections by following the VLDB style}

\subsection{The Multiple Hypothesis Testing Problem}

In \emph{statistical association testing}, the dependence of each pattern on the labels is quantified using its corresponding \emph{p-value}. In this context, the p-value is defined as the probability of measuring an association at least as extreme as the one observed in the data under the assumption that there is no real association present in the data-generating process. More precisely, let $H_{0}^{(i)}$ be the null hypothesis that the $i$-th pattern being examined is statistically independent of the class labels, $T^{(i)}$ the test-statistic chosen to evaluate association and $t^{(i)}$ the observed value of $T^{(i)}$. Assuming that larger values of $T^{(i)}$ indicate stronger dependence, the p-value is defined as $p_{i}=\mathrm{Pr}(\,T^{(i)} > t^{(i)} |  H_{0}^{(i)}\,)$. In practice, a pattern is considered to be significant if $p_{i} \le \alpha$, where $\alpha$ is called \emph{significance threshold}. 

When only one pattern is being tested, $\alpha$ coincides with the \emph{Type I error probability}; the probability of incorrectly rejecting a true null hypothesis. On the other hand, if we have a large number of patterns under study, statistical association testing becomes considerably more challenging because of the \emph{multiple hypothesis testing problem}. If there is a large number $D$ of patterns and those which satisfy $p_{i} \le \alpha$ are ruled as significant, then the probability that at least one out of the $D$ patterns will be wrongly deemed to be associated with the labels converges to $1$ at an exponential rate. That probability, commonly referred to as \emph{Family-Wise Error Rate (FWER)}, can be written mathematically as $\mathrm{FWER}=\mathrm{Pr}\left(\mathrm{FP} > 0\right)$, where $\mathrm{FP}$ denotes the number of false positives incurred by the testing procedure, i.e. the number of patterns erroneously considered to be dependent on the labels. 

When designing a multiple hypothesis testing procedure, upper bounding the FWER by a predefined value $\alpha$ is the most popular approach. Note that, from a data mining perspective, $\alpha$ must never be considered as a parameter to be optimized but, rather, as an application-dependent requirement set before observing the data. Intuitively, $\alpha$ controls the amount of ``risk'' the user is willing to take when searching for patterns in the data. Larger values of $\alpha$ corresponding to more risk but, also, enhanced ability to discover real signals.

Among all multiple hypothesis testing procedures which control the FWER, the \emph{Bonferroni correction} is the most commonly used. It is derived, and named, after the work in \cite{Bonferroni36} but was first used in \cite{dunn1959} . It is based on a simple principle. Assume we use a rule $p_{i}\le \delta$, where $\delta$ is the \emph{corrected significance threshold}, to determine which patterns are statistically significant. Then we can write the FWER as 
% $\mathrm{FWER} = \mathrm{Pr}\left(\cup_{i=1}^{D}{\set{\left[p_{i} \le \delta\right] | H_{0}^{(i)}}}\right)$,
$\mathrm{FWER} = \mathrm{Pr}(\,\bigcup_{i=1}^{D}\mathbbm{1}[p_{i} \le \delta]\,)$,
({\bf M: please check this is correct})
where $\mathbbm{1}[\bullet]$ denotes a function which evaluates to $1$ if its argument is true and to $0$ otherwise. By applying Boole's inequality we have
% $\mathrm{FWER} \le \sum_{i=1}^{D}\mathrm{Pr}\left(\set{\left[p_{i} \le \delta\right] | H_{0}^{(i)}}\right) \le \delta D$.
$\mathrm{FWER} \le \sum_{i=1}^{D}\mathrm{Pr}(\,\mathbbm{1}[p_{i} \le \delta]\,) \le \delta D$.
Therefore, setting $\delta = \alpha/D$ controls the FWER at significance level $\alpha$. Nevertheless, this correction has an important pitfall: If the number of tests $D$ is large enough, $\delta$ might be so small that the resulting testing procedure has virtually no statistical power to detect salient patterns in the data. While that poses a challenge in general, at first it appears to be an insurmountable hurdle for statistically sound data mining. In scenarios where $D$ increases exponentially fast with the database size, $D$ might be in the order of billions or even trillions and it seems unrealistic to think that any FWER-controlling procedure could have any  statistical power remaining after correcting the significance level. Furthermore, the multiple testing problem poses a huge computational challenge as well, since carrying out a number of significance tests exponentially growing with the database size is simply not feasible. 

\subsection{An Improved Bonferroni Correction for Discrete Test Statistics}

We first introduce an improved Bonferroni correction for discrete test statistics proposed by Tarone~\cite{Tarone}, which has profound implications for statistical significance testing in data mining. It uses the fact that, when discrete test statistics are employed, the corresponding p-values can only take a finite number of values. 

For instance, in our application, every p-value can be obtained from a $2 \times 2$ contingency table:
\begin{center}
	\begin{tabular}{|c|c|c|c|}
		\hline
		Variables & $S_{i}=1$ & $S_{i}=0$ & Row totals\\
		\hline
		$Y=1$ & $a_{i}$ & $n-a_{i}$ & $n$ \\
		\hline
		$Y=0$ & $x_{i}-a_{i}$ & $N+a_{i}-n-x_i$ & $N-n$ \\
		\hline
		Col totals & $x_{i}$ & $N-x_{i}$ & $N$ \\
		\hline
	\end{tabular}
\end{center}
Those are generally used to evaluate the strength of the association between two binary variables. In our case, the class labels $Y$ and a variable $S_{i}$ that indicates whether the $i$-th pattern is present or not for each of the $N$ objects in the database ($S_i = 1$ meaning that the $i$-th pattern exists in the object). In a given database, $N$ denotes the total number of objects, $n$ the number of objects with class label $Y = 1$, $x_{i}$ the number of objects containing the $i$-th pattern, and $a_{i}$ the number of objects with class label $Y = 1$ containing the $i$-th pattern. Without loss of generality, we assume that the class labels are encoded so that $n \le N-n$.  

When Fisher's exact test~\cite{FisherExactTest} is the test statistic of choice to obtain a p-value out of the $2 \times 2$ contingency table, the margins $x_{i}$, $n$ and $N$ are considered fixed. Consequently, the underlying data-generating model under the null hypothesis of statistical independence between $S_{i}$ and $Y$ is a hypergeometric random variable. Notice that when all margins are fixed, the table has only one degree of freedom left, which is why one can model the table as a one-dimensional count $a_{i}$.
% In fact, which of the four cell counts $a_{i}$, $n-a_{i}$, $x_{i}-a_{i}$ or $N+a_{i}-n-x_i$ is chosen is totally irrelevant, as all of them lead to the same probability distribution.
Mathematically, $\mathrm{Pr}\left(a_{i}=k | x_{i},n,N\right) = \binom{n}{k}\binom{N-n}{x_{i}-k} / \binom{N}{x_{i}}$ with support on $a_{i,\mathrm{min}} \leq k \leq a_{i,\mathrm{max}}$, $a_{i,\mathrm{min}}=\max(0,x_{i}+n-N)$ and $a_{i,\mathrm{max}}=\min(n,x_{i})$. If for a given pattern we observe $a_{i}=\gamma$, the corresponding \emph{one-tailed} p-value can be obtained as $p_{i}(\gamma) = \min \left(\Phi_{\mathrm{l}}(\gamma),\Phi_{\mathrm{r}}(\gamma)\right)$, where we define $\Phi_{\mathrm{l}}(\gamma)=\sum_{k=a_{i,\mathrm{min}}}^{\gamma}{\mathrm{Pr}\left( a_{i}=k | x_{i},n,N \right)}$ and $\Phi_{\mathrm{r}}(\gamma)=\sum_{k=\gamma}^{a_{i,\mathrm{max}}}{\mathrm{Pr}\left( a_{i}=k | x_{i},n,N \right)}$ as the left and right tails of the hypergeometric distribution, respectively. To get a \emph{two-tailed} p-value, one can simply double the one-tailed p-value.

Since $a_{i}$ can only take $a_{i,\mathrm{max}} - a_{i,\mathrm{min}} +1$ different values, the corresponding p-values $p_{i}(a_{i})$ are also finitely many. Hence, there exists a {\em minimum attainable p-value} defined as $\Psi(x_{i},n,N) = \min\set{p_{i}(\gamma) | a_{i,\mathrm{min}} \leq \gamma \leq a_{i,\mathrm{max}}}$. As $n$ and $N$ depend only on the labels and are therefore fixed for all patterns, we abbreviate $\Psi(x_{i},n,N)$ as $\Psi(x_{i})$ in the rest of the paper. Given a tentative corrected significance threshold $\delta$
% and just based on the margins $x$, $n$ and $N$ of the 2x2 contingency table,
one can know that all patterns for which $\Psi(x_{i}) > \delta$ have no chance of being significant and can be pruned from the search space. We will refer to those patterns as \emph{untestable}, while those satisfying $\Psi(x_{i}) \le \delta$ will be said to be \emph{testable}. Even more importantly, because those patterns can never be significant, they do not need to be included in the Bonferroni correction factor. Precisely, let $\mathcal{I}_{T}(\delta)$ be the set of patterns testable at level $\delta$, that is, $\mathcal{I}_{T}(\delta) = \left\{i \in \left\{1,\hdots,D\right\} | \Psi(x_{i}) \le \delta \right\}$ and $m(\delta)=\left\vert \mathcal{I}_{T}(\delta) \right\vert$. Then, following the same steps used to derive the Bonferroni correction, one can prove that $\mathrm{FWER} \le \delta m(\delta)$. Thus, an improved corrected significance threshold can be found as $\delta^{*} = \max\set{\delta | \delta m(\delta) \le \alpha}$. Since $m(\delta) \ll D$ in most real-world datasets, this improvement can bring a drastic increase in statistical power.

One fundamental observation, not emphasised neither in \cite{Tarone} nor \cite{TeradaPNAS}, is that it is essential that the model under the null hypothesis for Fisher's exact test is a probability distribution conditioned on the table marginals. Otherwise, the whole method would not be mathematically sound. Since $\Psi(x_{i})$ conveys information about $x_{i}$, $n$ and $N$, if the distribution of the test statistic under the null hypothesis was not conditional on the margins, knowledge about $\Psi(x_{i})$ could potentially distort the distribution of null p-values due to ``information leaking''. Intuitively, one relies on using test statistics for which evaluating the minimum attainable p-value does not involve any magnitudes modelled as random variables under the null hypothesis or, if it does, those must be provably statistically independent of the test statistic from which the p-values are computed.

This improved Bonferroni correction, as proposed in \cite{Tarone}, would require computing $\Psi(x_{i})$ for each pattern in order to evaluate $m(\delta)$ as many times as needed in a linear search. Needless to say, in a data mining context, such approach is unfeasible except for toy examples, as it would require mining and computing the support of every single pattern in the dataset. The computational unfeasibility of the original method resulted in it being largely ignored by the data mining community until until the 2013 breakthrough paper by Terada et al.~\cite{TeradaPNAS}. There, the authors propose the Limitless-Arity Multiple-testing Procedure (LAMP), a branch-and-bound algorithm which is able to apply the method described in~\cite{Tarone} to data mining problems of the form considered in this paper.

\subsection{Addressing Dependence Between Test Statistics}

In data mining settings such as the ones described in this work, it is intuitively clear that a large amount of patterns will in fact be part of greater patterns and, hence, complex correlation structures involving the different $D$ test statistics will exist. However, neither \cite{Tarone} nor \cite{TeradaPNAS} address how to model the correlation structure between test statistics. 

Ideally, the problem to be solved is $\delta^{*} = \max\set{\delta | \mathrm{FWER}(\delta) \le \alpha}$. Nonetheless, since evaluating $\mathrm{FWER}(\delta)$ is a costly task, all methods exposed so far use some quantity as a surrogate upper bound of the FWER instead. For instance, Bonferroni's correction corresponds to using $f(\delta) = \delta D$, whereas the method described in \cite{Tarone} and implemented by \cite{TeradaPNAS} employs $f(\delta) = \delta m(\delta)$. In both cases, those upper bounds completely neglect the dependence between test statistics. Thus, the resulting upper bounds are quite loose, leading to over-conservative procedures with a significant loss of statistical power. It is therefore of great interest to develop algorithms to solve the original problem without using any upper bound on the FWER as a surrogate. 

By definition, the FWER can also be expressed as $\mathrm{FWER}(\delta) = \mathrm{CDF}_{\Omega}(\delta)$ where $\Omega$ is the Random Variable $\Omega = \min\set{p_{i} | i \in \mathcal{K}} | H_{0}^{\mathcal{K}}$, $H_{0}^{\mathcal{K}} = \cap_{i \in \mathcal{K}}{H_{0}^{(i)}}$ and $\mathcal{K}$ is the set of true null hypotheses. Under a certain technical condition known as the subset pivotality condition, the FWER can also be obtained as the CDF of the random variable $\Omega^{\prime} = \min\set{p_{i} | i \in \set{1,\hdots,D}} | \mathbf{H}_{0}$, with $\mathbf{H}_{0} = \cap_{\set{1,\hdots,D}}{H_{0}^{(i)}}$, which is simpler as it does not depend on the (unknown) ground truth. Since most often there is no analytic formula available for the distribution of $\Omega^{\prime}$, nor its CDF, one resorts to resampling methods to approximate it.

In the context of statistical association testing, a permutation based resampling scheme proposed by Westfall and Young \cite{WYBook} is one of the most popular approaches. The idea is as follows: if one has to test the association of D random variables $\left\{S_{i}\right\}_{i=1}^{D}$ with another random variable $Y$, a simple way of generating samples of the p-values under the global null (i.e. to generate samples of $\Omega^{\prime}$) is by randomly shuffling (permuting) the observations of $Y$ with respect to those of the random variables $\left\{S_{i}\right\}_{i=1}^{D}$. The permuted datasets obtained that way are effectively samples of the distribution $\mathrm{Pr}\left(\left\{S_{i}\right\}_{i=1}^{D}\right)\mathrm{Pr}(Y)$ and, therefore, correspond to samples obtained from the global null hypothesis that all variables $\left\{S_{i}\right\}_{i=1}^{D}$ are independent of $Y$. Those can then be used to obtain samples from $\mathrm{PDF}(\Omega^{\prime})$ by computing the respective p-values and taking the minimum across all patterns in the database, i.e. $p_{\mathrm{min}}= \min\set{\tilde{p}_{i} | i \in \set{1,\hdots,D}} \sim \mathrm{PDF}(\Omega^{\prime})$, where $\tilde{p}_{i}$ is the p-value resulting from evaluating the association between $S_{i}$ and one realisation of the permuted class labels $\widetilde{Y}$.

While conceptually simple, the Westfall-Young permutation scheme can be extremely computationally demanding. Generating a single sample from $\mathrm{PDF}(\Omega^{\prime})$ naively requires computing the p-values corresponding to all $D$ patterns using a specific permuted version of the class labels, $\widetilde{Y}$. Besides, to get a reasonably good empirical approximation to $\mathrm{FWER}(\delta) = \mathrm{CDF}_{\Omega^{\prime}}(\delta)$, one needs several samples $p_{\mathrm{min}}  \sim \mathrm{PDF}(\Omega^{\prime})$. As it will be shown in the experiments section, a number of samples in the order of $J=10^{3}$ or $J=10^{4}$ is needed to get reliable results. 

In \cite{TeradaIEEE} Terada et al.~were the first to propose an algorithm, called FastWY, which again exploits the discreteness . 
of test statistics to reduce the computational burden which the Westfall-Young permutation-based procedure entails.

Both the LAMP algorithm in \cite{TeradaPNAS} and the FastWY algorithm in \cite{TeradaIEEE} are based on using a surrogate lower bound $\hat{\Psi}(x_{i})$ for the minimum attainable p-value function which is monotonically decreasing in $[0,N]$. They define $\hat{\Psi}(x_{i})$ in such a way\footnote{$\hat{\Psi}(x_{i}) = \begin{cases}\Psi(x_{i}) & 0 \leq x_{i} \leq n \\1 \Big/ \binom{N}{n} & n < x_{i} \leq N \\\end{cases}$} that all patterns for which $x_{i}>n$ are considered to be testable even if that is not necessarily the case. In other words, with their approach one would fetch a set of ``potentially testable'' patterns $\hat{\mathcal{I}}_{T}(\delta) = \left\{i \in \left\{1,\hdots,D\right\} | \hat{\Psi}(x_{i}) \le \delta \right\}$ satisfying $\mathcal{I}_{T}(\delta) \subset \hat{\mathcal{I}}_{T}(\delta)$. Nonetheless, as a result of decreasing monotonicity of $\hat{\Psi}$, they introduce $\sigma(\delta)=\inf \left\{x_i | \hat{\Psi}(x_{i}) \le \delta \right\}$ which enables them to rewrite $\hat{\mathcal{I}}_{T}(\delta)$ as $\hat{\mathcal{I}}_{T}(\sigma(\delta)) = \left\{i \in \left\{1,\hdots,D\right\} | x_{i} \ge \sigma(\delta) \right\}$. This new formulation is important because, unlike the set $\mathcal{I}_{T}(\delta)$ defined in \cite{Tarone}, $\hat{\mathcal{I}}_{T}(\sigma(\delta))$ can be readily seen to correspond to an instance of \emph{frequent pattern mining with support $\sigma(\delta)$}, a well studied problem in data mining.

Now, if the p-values for all patterns in $\hat{\mathcal{I}}_{T}(\sigma)$ are known and $p_{\mathrm{min}}=\min\set{\tilde{p}_{i} | i \in \hat{\mathcal{I}}_{T}(\sigma)} \le \hat{\Psi}(\sigma)$ then no pattern in $\set{1,\hdots,D} \setminus \hat{\mathcal{I}}_{T}(\sigma)$ can possibly attain a p-value smaller than $p_{\mathrm{min}}$ and the search can be stopped early.

FastWY exploits that property to sample from $\mathrm{PDF}(\Omega^{\prime})$ without having to explicitly compute all $D$ p-values. It is based on a decremental search scheme starting with $\sigma=n$. First, a frequent pattern miner is used as a black box to retrieve the set $\hat{\mathcal{I}}_{T}(\sigma)$. Then, the p-values $\tilde{p}_{i}$ are computed $\forall i \in \hat{\mathcal{I}}_{T}(\sigma)$ and $p_{\mathrm{min}}=\min\set{\tilde{p}_{i} | i \in \hat{\mathcal{I}}_{T}(\sigma)}$ is evaluated. If $p_{\mathrm{min}} \le \hat{\Psi}(\sigma)$, no other pattern would be able to make $p_{\mathrm{min}}$ smaller and, therefore, $p_{\mathrm{min}}$ constitutes an exact sample from $\mathrm{PDF}(\Omega^{\prime})$. On the contrary, if $p_{\mathrm{min}} > \hat{\Psi}(\sigma)$, $\sigma$ is decreased by one unit and the whole procedure is repeated until the condition $p_{\mathrm{min}} \le \hat{\Psi}(\sigma)$ is satisfied.

If $J$ permutations are needed to empirically estimate the FWER, the procedure has be to repeated $J$ times. That includes the whole sequence of frequent mining problems needed to retrieve the sets $\hat{\mathcal{I}}_{T}(\sigma)$ for each value of $\sigma$ used throughout the decremental search. Given the usual range of values for $J$, such an approach is just as unfeasible in practice as the original brute force baseline.

Interestingly, careful inspection of the code kindly shared by the authors in their website reveals that the actual implementation of the algorithm is different from the description in \cite{TeradaIEEE}. Indeed, to alleviate the inadmissible burden of repeating the whole frequent pattern mining process $J$ times, the authors resort to storing the realisations of the variables $S_{i} \; \forall i \in \hat{\mathcal{I}}_{T}(\sigma)$ and every value of $\sigma$ explored during the decremental search. Clearly, this decision corresponds to a drastic trade-off between runtime and memory usage since, as we will show empirically, there exist many databases for which the amount of information to be stored when following that approach is too large to fit even in large servers equipped with 512GB of RAM. Furthermore, we will also demonstrate that the algorithm resulting from trading off memory in exchange for runtime is still slow even for mid-sized datasets and can be greatly improved.

When referring to the FastWY algorithm in \cite{TeradaIEEE} throughout the remaining of this paper, we mean the runtime-optimised version of the algorithm, given that the algorithm exactly as described in \cite{TeradaIEEE} simply cannot be run in a reasonable amount of time.


==> background2.tex <==
\section{Background}
\label{sec:background}

\subsection{The Multiple Hypothesis Testing Problem}

In \emph{statistical association testing}, the dependence of each pattern on the labels is quantified using its corresponding \emph{p-value}. In this context, the p-value is defined as the probability of measuring an association at least as extreme as the one observed in the data under the assumption that there is no real association present in the data-generating process. More precisely, let $H_{0}^{(i)}$ be the null hypothesis that the $i$-th pattern being examined is statistically independent of the class labels, $T^{(i)}$ the test-statistic chosen to evaluate association and $t^{(i)}$ the observed value of $T^{(i)}$. Assuming that larger values of $T^{(i)}$ indicate stronger dependence, the p-value is defined as $p_{i}=\mathrm{Pr}(\,T^{(i)} > t^{(i)} |  H_{0}^{(i)}\,)$. In practice, a pattern is considered to be significant if $p_{i} \le \alpha$, where $\alpha$ is called \emph{significance threshold}. 

When only one pattern is being tested, $\alpha$ coincides with the \emph{Type I error probability}; the probability of incorrectly rejecting a true null hypothesis. On the other hand, if we have a large number of patterns under study, statistical association testing becomes considerably more challenging because of the \emph{multiple hypothesis testing problem}. If there is a large number $D$ of patterns and those which satisfy $p_{i} \le \alpha$ are ruled as significant, then the probability that at least one out of the $D$ patterns will be wrongly deemed to be associated with the labels converges to $1$ at an exponential rate. That probability, commonly referred to as \emph{Family-Wise Error Rate (FWER)}, can be written mathematically as $\mathrm{FWER}=\mathrm{Pr}\left(\mathrm{FP} > 0\right)$, where $\mathrm{FP}$ denotes the number of false positives incurred by the testing procedure, i.e. the number of patterns erroneously considered to be dependent on the labels. 

Ideally, the problem to be solved is
\[
	\delta^{*} = \max\set{\delta | \mathrm{FWER}(\delta) \le \alpha},
\]
where $\delta$ is the \emph{corrected significance threshold} to determine which patterns are statistically significant and 
$\mathrm{FWER}(\delta)$ is the resulting FWER of that procedure. Nonetheless, since evaluating $\mathrm{FWER}(\delta)$ is a costly task, all methods exposed so far use some quantity as a surrogate upper bound of the FWER instead. For instance, one of the most popular correction methods, the {\em Bonferroni correction}~\cite{Bonferroni36}, corresponds to using $f(\delta) = \delta D$.
% whereas the method described in \cite{Tarone} and implemented by \cite{TeradaPNAS} employs $f(\delta) = \delta m(\delta)$.
However, in data mining settings, it is intuitively clear that a large amount of patterns will in fact be a part of its super  patterns. Hence complex correlation structures involving the different $D$ test statistics will exist.
%However, neither \cite{Tarone} nor \cite{TeradaPNAS} address how to model the correlation structure between test statistics. 
Since the upper bound by Bonferroni correction completely neglects the dependence between test statistics, the resulting upper bounds are quite loose, leading to over-conservative procedures with a significant loss of statistical power. It is therefore of great interest to develop algorithms to solve the original problem without using any upper bound on the FWER as a surrogate. 

By definition, the FWER can be expressed as $\mathrm{FWER}(\delta) = \mathrm{CDF}_{\Omega}(\delta)$, where $\Omega$ is the random variable $\Omega = \min\{\,p_{i} \mid i \in \mathcal{K}\,\} \mid H_{0}^{\mathcal{K}}$, $H_{0}^{\mathcal{K}} = \bigcap_{i \in \mathcal{K}}{H_{0}^{(i)}}$ and $\mathcal{K}$ is the set of true null hypotheses. Under a certain technical condition known as the subset pivotality condition, the FWER can also be obtained as the CDF of the random variable $\Omega^{\prime} = \min\{\,p_{i} \mid i \in \{\,1,\hdots,D\,\}\,\} \mid \mathbf{H}_{0}$, with $\mathbf{H}_{0} = \bigcap_{\set{1,\hdots,D}}{H_{0}^{(i)}}$, which is simpler as it does not depend on the (unknown) ground truth. Since most often there is no analytic formula available for the distribution of $\Omega^{\prime}$, nor its CDF, one resorts to resampling methods to approximate it.

When designing a multiple hypothesis testing procedure, upper bounding the FWER by a predefined value $\alpha$ is the most popular approach. Note that, from a data mining perspective, $\alpha$ must never be considered as a parameter to be optimized but, rather, as an application-dependent requirement set before observing the data. Intuitively, $\alpha$ controls the amount of ``risk'' the user is willing to take when searching for patterns in the data. Larger values of $\alpha$ corresponding to more risk but, also, enhanced ability to discover real signals.

\subsection{Westfall-Young Permutation-based\\ hypothesis testing}

In the context of statistical association testing, a permutation based resampling scheme proposed by Westfall and Young \cite{WYBook} is one of the most popular approaches to account for correlation structures. The idea is as follows: if one has to test the association of $D$ random variables $\left\{S_{i}\right\}_{i=1}^{D}$ with another random variable $Y$, a simple way of generating samples of the p-values under the global null (i.e.~to generate samples of $\Omega^{\prime}$) is by randomly shuffling (permuting) of the observations of $Y$ with respect to those of the random variables $\left\{S_{i}\right\}_{i=1}^{D}$. The permuted datasets obtained that way are effective samples of the distribution $\mathrm{Pr}(\,\{S_{i}\}_{i=1}^{D}\,)\mathrm{Pr}(Y)$ and, therefore, correspond to samples obtained from the global null hypothesis that all variables $\left\{S_{i}\right\}_{i=1}^{D}$ are independent of $Y$. Those can then be used to obtain samples from $\mathrm{PDF}(\Omega^{\prime})$ by computing the respective p-values and taking the minimum across all patterns in the database, i.e.~$p_{\mathrm{min}}= \min_{i \in \set{1,\hdots,D}} \tilde{p}_{i} \sim \mathrm{PDF}(\Omega^{\prime})$, where $\tilde{p}_{i}$ is the p-value resulting from evaluating the association between $S_{i}$ and one realization of the permuted class labels $\widetilde{Y}$.

While conceptually simple, the Westfall-Young permutation scheme can be extremely computationally demanding. Generating a single sample from $\mathrm{PDF}(\Omega^{\prime})$ naively requires computing the p-values corresponding to all $D$ patterns using a specific permuted version of the class labels, $\widetilde{Y}$. Besides, to get a reasonably good empirical approximation to $\mathrm{FWER}(\delta) = \mathrm{CDF}_{\Omega^{\prime}}(\delta)$, one needs several samples $p_{\mathrm{min}}  \sim \mathrm{PDF}(\Omega^{\prime})$. As it will be shown in the experiments section, a number of samples in the order of $J=10^{3}$ or $J=10^{4}$ is needed to get reliable results. 

\subsection{State-of-the-art in Significant Pattern\\ Mining}

Terada et al.~\cite{TeradaIEEE} were the first to propose an efficient algorithm, called FastWY, which enables us to use Westfall-Young permutation in the setting of itemset mining.
%were the first to propose an algorithm, called FastWY, which again exploits the discreteness of test statistics to reduce the computational burden which the Westfall-Young permutation-based procedure entails.
The method uses inherent properties of discrete test statistics and succeeded to reduce the computational burden which the Westfall-Young permutation-based procedure entails. In the following we introduce the algorithm since we share the same problem setting and the key concept of the minimum attainable p-value.

%We first introduce an improved Bonferroni correction for discrete test statistics proposed by Tarone~\cite{Tarone}, which has profound implications for statistical significance testing in data mining. It uses the fact that, when discrete test statistics are employed, the corresponding p-values can only take a finite number of values. 

In pattern mining, every p-value can be obtained from a $2 \times 2$ contingency table:
\begin{center}
	\begin{tabular}{|c|c|c|c|}
		\hline
		Variables & $S_{i}=1$ & $S_{i}=0$ & Row totals\\
		\hline
		$Y=1$ & $a_{i}$ & $n-a_{i}$ & $n$ \\
		\hline
		$Y=0$ & $x_{i}-a_{i}$ & $N+a_{i}-n-x_i$ & $N-n$ \\
		\hline
		Col totals & $x_{i}$ & $N-x_{i}$ & $N$ \\
		\hline
	\end{tabular}
\end{center}
This is generally used to evaluate the strength of the association between two binary variables. In our case, the class labels $Y$ and a variable $S_{i}$ that indicates whether the $i$-th pattern is present or not for each of the $N$ objects in the database ($S_i = 1$ meaning that the $i$-th pattern exists in the object). In a given database, $N$ denotes the total number of objects, $n$ the number of objects with class label $Y = 1$, $x_{i}$ the number of objects containing the $i$-th pattern, and $a_{i}$ the number of objects with class label $Y = 1$ containing the $i$-th pattern. Without loss of generality, we assume that the class labels are encoded so that $n \le N-n$.  

Let us use {\em Fisher's exact test}~\cite{FisherExactTest} to compute the test statistic, which is the standard test to obtain a p-value out of the $2 \times 2$ contingency table.
The underlying data-generating model under the null hypothesis of statistical independence between $S_{i}$ and $Y$ is a hypergeometric random variable. Notice that when all marginals $x_{i}$, $n$, and $N$ are considered fixed, the table has only one degree of freedom left, which is why one can model the table as a one-dimensional count $a_{i}$.
% In fact, which of the four cell counts $a_{i}$, $n-a_{i}$, $x_{i}-a_{i}$ or $N+a_{i}-n-x_i$ is chosen is totally irrelevant, as all of them lead to the same probability distribution.
Mathematically, $\mathrm{Pr}\left(a_{i}=k | x_{i},n,N\right) = \binom{n}{k}\binom{N-n}{x_{i}-k} / \binom{N}{x_{i}}$ with support on $a_{i,\mathrm{min}} \leq k \leq a_{i,\mathrm{max}}$, $a_{i,\mathrm{min}}=\max\{0,x_{i}+n-N\}$ and $a_{i,\mathrm{max}}=\min\{n,x_{i}\}$. If for a given pattern we observe $a_{i}=\gamma$, the corresponding \emph{one-tailed} p-value can be obtained as $p_{i}(\gamma) = \min \{\Phi_{\mathrm{l}}(\gamma),\Phi_{\mathrm{r}}(\gamma)\}$, where we define $\Phi_{\mathrm{l}}(\gamma)=\sum_{k=a_{i,\mathrm{min}}}^{\gamma}{\mathrm{Pr}\left( a_{i}=k | x_{i},n,N \right)}$ and $\Phi_{\mathrm{r}}(\gamma)=\sum_{k=\gamma}^{a_{i,\mathrm{max}}}{\mathrm{Pr}\left( a_{i}=k | x_{i},n,N \right)}$ as the left and right tails of the hypergeometric distribution, respectively. To get a \emph{two-tailed} p-value, one can simply double the one-tailed p-value.

Since $a_{i}$ can only take $a_{i,\mathrm{max}} - a_{i,\mathrm{min}} +1$ different values, the corresponding p-values $p_{i}(a_{i})$ are also finitely many. Hence, there exists a {\em minimum attainable p-value} defined as $\Psi(x_{i},n,N) = \min\set{p_{i}(\gamma) | a_{i,\mathrm{min}} \leq \gamma \leq a_{i,\mathrm{max}}}$. As $n$ and $N$ depend only on the labels and are therefore fixed for all patterns, we abbreviate $\Psi(x_{i},n,N)$ as $\Psi(x_{i})$ in the rest of the paper.
For a given $\delta$, we denote by $\mathcal{I}_{T}(\delta)$ the set $\{\,i \in \left\{1,\hdots,D\right\} \mid \Psi(x_{i}) \le \delta \,\}$.

The key to the FastWY algorithm is to use this minimum attainable p-value, and the algorithm requires it to be monotonically decreasing in $[0,N]$. To achieve this requirement, FastWY uses a surrogate lower bound $\hat{\Psi}(x_{i})$ defined as
% Both the LAMP algorithm in \cite{TeradaPNAS} and the FastWY algorithm in \cite{TeradaIEEE} are based on using a surrogate lower bound $\hat{\Psi}(x_{i})$ for the minimum attainable p-value function which is monotonically decreasing in $[0,N]$.
\begin{flalign*}
\hat{\Psi}(x_{i}) = \begin{cases}\Psi(x_{i}) & 0 \leq x_{i} \leq n, \\1 \big/ \binom{N}{n} & n < x_{i} \leq N \\\end{cases}
\end{flalign*}
and define $\hat{\mathcal{I}}_{T}(\delta) = \{\,i \in \left\{1,\hdots,D\right\} \mid \hat{\Psi}(x_{i}) \le \delta\,\}$, which always satisfies $\mathcal{I}_{T}(\delta) \subset \hat{\mathcal{I}}_{T}(\delta)$.
% so that all patterns with $x_{i}>n$ are considered to be testable even if that is not necessarily the case. In other words, with their approach one would fetch a set of ``potentially testable'' patterns $\hat{\mathcal{I}}_{T}(\delta) = \{\,i \in \left\{1,\hdots,D\right\} \mid \hat{\Psi}(x_{i}) \le \delta\,\}$ satisfying $\mathcal{I}_{T}(\delta) \subset \hat{\mathcal{I}}_{T}(\delta)$. Nonetheless, 
As a result of monotonicity of $\hat{\Psi}$, we can rewrite $\hat{\mathcal{I}}_{T}(\delta)$ as $\hat{\mathcal{I}}_{T}(\sigma(\delta)) = \{\,i \in \left\{1,\hdots,D\right\} \mid x_{i} \ge \sigma(\delta)\,\}$ using $\sigma(\delta)=\inf \{\,x_i \mid \hat{\Psi}(x_{i}) \le \delta\,\}$. This new formulation is important because
%unlike the set $\mathcal{I}_{T}(\delta)$ defined in \cite{Tarone}, 
$\hat{\mathcal{I}}_{T}(\sigma(\delta))$ can be readily seen to correspond to an instance of \emph{frequent pattern mining with support $\sigma(\delta)$}, a well studied problem in data mining.

Here the key property used by FastWY is as follows: If the p-values for all patterns in $\hat{\mathcal{I}}_{T}(\sigma)$ are known and $p_{\mathrm{min}}=\min\set{\tilde{p}_{i} | i \in \hat{\mathcal{I}}_{T}(\sigma)} \le \hat{\Psi}(\sigma)$, no pattern in $\set{1,\hdots,D} \setminus \hat{\mathcal{I}}_{T}(\sigma)$ can possibly attain a p-value smaller than $p_{\mathrm{min}}$ and the search can be stopped early.

FastWY exploits that property to sample from $\mathrm{PDF}(\Omega^{\prime})$ without having to explicitly compute all $D$ p-values. It is based on a decremental search scheme starting with $\sigma=n$. First, a frequent pattern miner is used as a black box to retrieve the set $\hat{\mathcal{I}}_{T}(\sigma)$. Then, the p-values $\tilde{p}_{i}$ are computed for all $i \in \hat{\mathcal{I}}_{T}(\sigma)$ and $p_{\mathrm{min}}=\min\set{\tilde{p}_{i} | i \in \hat{\mathcal{I}}_{T}(\sigma)}$ is evaluated. If $p_{\mathrm{min}} \le \hat{\Psi}(\sigma)$, no other pattern would be able to make $p_{\mathrm{min}}$ smaller and, therefore, $p_{\mathrm{min}}$ constitutes an exact sample from $\mathrm{PDF}(\Omega^{\prime})$. On the contrary, if $p_{\mathrm{min}} > \hat{\Psi}(\sigma)$, $\sigma$ is decreased by one unit and the whole procedure is repeated until the condition $p_{\mathrm{min}} \le \hat{\Psi}(\sigma)$ is satisfied.

If $J$ permutations are needed to empirically estimate the FWER, the procedure has be to repeated $J$ times. That includes the whole sequence of frequent mining problems needed to retrieve the sets $\hat{\mathcal{I}}_{T}(\sigma)$ for each value of $\sigma$ used throughout the decremental search. Given the usual range of values for $J$, such an approach is just as unfeasible in practice as the original brute force baseline.

Interestingly, careful inspection of the code kindly shared by the authors in their website reveals that the actual implementation of the algorithm is different from the description in \cite{TeradaIEEE}. Indeed, to alleviate the inadmissible burden of repeating the whole frequent pattern mining process $J$ times, the authors resort to storing the realisations of the variables $S_{i}$ for all $i \in \hat{\mathcal{I}}_{T}(\sigma)$ and every value of $\sigma$ explored during the decremental search. Clearly, this decision corresponds to a drastic trade-off between runtime and memory usage since, as we will show empirically, there exist many databases for which the amount of information to be stored when following that approach is too large to fit even in large servers equipped with 512GB of RAM. Furthermore, we will also demonstrate that the algorithm resulting from trading off memory in exchange for runtime is still slow even for mid-sized datasets and can be greatly improved.

When referring to the FastWY algorithm in \cite{TeradaIEEE} throughout the remaining of this paper, we mean the runtime optimized version of the algorithm, given that the algorithm exactly as described in \cite{TeradaIEEE} simply cannot be run in a reasonable amount of time.


==> multipletesting.tex <==
\section{The Multiple Hypothesis Testing Problem}
\label{sec:multipletesting}

In \emph{statistical association testing}, the dependence of each pattern on the labels is quantified using its corresponding \emph{p-value}. In this context, the p-value is defined as the probability of measuring an association at least as extreme as the one observed in the data under the assumption that there is no real association present in the data-generating process. More precisely, let $H_{0}^{(i)}$ be the null hypothesis that the $i$-th pattern being examined is statistically independent of the class labels, $T^{(i)}$ the test-statistic chosen to evaluate association and $t^{(i)}$ the observed value of $T^{(i)}$. Assuming that larger values of $T^{(i)}$ indicate stronger dependence, the p-value is defined as $p_{i}=\mathrm{Pr}(\,T^{(i)} > t^{(i)} |  H_{0}^{(i)}\,)$. In practice, a pattern is considered to be significant if $p_{i} \le \alpha$, where $\alpha$ is called \emph{significance threshold}. 

When only one pattern is being tested, $\alpha$ coincides with the \emph{Type I error probability}; the probability of incorrectly rejecting a true null hypothesis. On the other hand, if we have a large number of patterns under study, statistical association testing becomes considerably more challenging because of the \emph{multiple hypothesis testing problem}. If there is a large number $D$ of patterns and those which satisfy $p_{i} \le \alpha$ are ruled as significant, the probability that at least one out of the $D$ patterns will be wrongly deemed to be associated with the labels converges to $1$ at an exponential rate. That probability, commonly referred to as \emph{Family-Wise Error Rate (FWER)}, can be written mathematically as $\mathrm{FWER}=\mathrm{Pr}\left(\mathrm{FP} > 0\right)$, where $\mathrm{FP}$ denotes the number of false positives incurred by the testing procedure, i.e. the number of patterns erroneously considered to be dependent on the labels. 

When designing a multiple hypothesis testing procedure, upper bounding the FWER by a predefined value $\alpha$ is the most popular approach. Note that, from a data mining perspective, $\alpha$ must never be considered as a parameter to be optimized but, rather, as an application-dependent requirement set before observing the data. Intuitively, $\alpha$ controls the amount of ``risk'' the user is willing to take when searching for patterns in the data. Larger values of $\alpha$ corresponding to more risk but, also, enhanced ability to discover real signals.

Among all multiple hypothesis testing procedures which control the FWER, the \emph{Bonferroni correction} is the most commonly used. It is derived, and named, after the work in \cite{Bonferroni36} but was first used in \cite{dunn1959} . It is based on a simple principle. Assume we use a rule $p_{i}\le \delta$, where $\delta$ is the \emph{corrected significance threshold}, to determine which patterns are statistically significant. Then we can write the FWER as $\mathrm{FWER} = \mathrm{Pr}\left(\cup_{i=1}^{D}\left[p_{i} \le \delta\right | H_{0}^{(i)}]\right)$, where $\mathbbm{1}[\bullet]$ denotes a function which evaluates to $1$ if its argument is true and to $0$ otherwise. By applying Boole's inequality we have that $\mathrm{FWER} \le \sum_{i=1}^{D}\mathrm{Pr}\left(\left[p_{i} \le \delta\right | H_{0}^{(i)}]\right) \le \delta D$. Therefore, setting $\delta = \alpha/D$ controls the FWER at significance level $\alpha$. Nevertheless, this correction has an important pitfall: if the number of tests $D$ is large enough, $\delta$ might be so small that the resulting testing procedure has virtually no statistical power to detect salient patterns in the data. While that poses a challenge in general, at first it appears to be an insurmountable hurdle for statistically sound data mining. In scenarios where $D$ increases exponentially fast with the database size, $D$ might be in the order of billions or even trillions and it seems unrealistic to think that any FWER-controlling procedure could have any  statistical power remaining after correcting the significance level. Furthermore, the multiple testing problem poses a huge computational challenge as well, since carrying out a number of significance tests exponentially growing with the database size is simply not feasible. 



==> relatedwork.tex <==
\section{Related Work}
\label{sec:related_work}


As a consequence of all the aforementioned difficulties, assessing the statistical significance of patterns mined in large databases while correcting for multiple hypothesis testing was considered to be a hopeless endeavor until the 2013 breakthrough paper by Terada et al.~\cite{TeradaPNAS}. There, the authors propose the Limitless-Arity Multiply-testing Procedure (LAMP), a branch-and-bound algorithm which is able to apply the method described in~\cite{Tarone} to data mining problems of the form considered in this paper. 

\subsection*{An improved Bonferroni correction for discrete data}

\begin{table}[ht]
\centering
	\begin{tabular}{|c|c|c|c|}
		\hline
		Variables & $S_{i}=1$ & $S_{i}=0$ & Row totals\\
		\hline
		$Y=1$ & $a_{i}$ & $n-a_{i}$ & $n$ \\
		\hline
		$Y=0$ & $x_{i}-a_{i}$ & $N+a_{i}-n-x_i$ & $N-n$ \\
		\hline
		Col totals & $x_{i}$ & $N-x_{i}$ & $N$ \\
		\hline
	\end{tabular}
\caption{2x2 contingency table corresponding to the $i$-th pattern being tested.}
\label{tab:contingency_table}
\end{table}

The original idea proposed by Tarone in \cite{Tarone} uses the fact that, when discrete test statistics are employed, the corresponding p-values can only take a finite number of values. For instance, in our application, all p-values can be obtained from $2 \times 2$ contingency tables as the one shown in Table~\ref{tab:contingency_table}, where $N$ is the number of objects in a given database and $n$ is the number of objects such that the class labels $Y = 0$. Without loss of generality, we assume that the class labels are encoded so that $n \le N-n$. Those are used to evaluate the strength of the association between two binary variables: the class labels $Y$ and a variable $S_{i}$ which indicates if the $i$-th pattern is present in each of the $N$ objects in the database ($S_i = 1$ means that the $i$-th pattern exists). When Fisher's exact test~\cite{FisherExactTest} is the test statistic of choice to obtain a p-value out of the $2 \times 2$ contingency table, the margins $x_{i}$, $n$ and $N$ are considered to be fixed. Consequently, the underlying data-generating model under the null hypothesis of statistical independence between $S_{i}$ and $Y$ is a hypergeometric random variable. Notice that when all margins are fixed, the table has only one degree of freedom left, which is why one can model the table as a one-dimensional count $a_{i}$.
% In fact, which of the four cell counts $a_{i}$, $n-a_{i}$, $x_{i}-a_{i}$ or $N+a_{i}-n-x_i$ is chosen is totally irrelevant, as all of them lead to the same probability distribution.
Mathematically, $\mathrm{Pr}\left(a_{i}=k | x_{i},n,N\right) = \binom{n}{k}\binom{N-n}{x_{i}-k} / \binom{N}{x_{i}}$ with support on $a_{i,\mathrm{min}} \leq k \leq a_{i,\mathrm{max}}$, $a_{i,\mathrm{min}}=\max(0,x_{i}+n-N)$ and $a_{i,\mathrm{max}}=\min(n,x_{i})$. If for a given pattern we observe $a_{i}=\gamma$, the corresponding \emph{one-tailed} p-value can be obtained as $p_{i}(\gamma) = \min \left(\Phi_{\mathrm{l}}(\gamma),\Phi_{\mathrm{r}}(\gamma)\right)$, where we define $\Phi_{\mathrm{l}}(\gamma)=\sum_{k=a_{i,\mathrm{min}}}^{\gamma}{\mathrm{Pr}\left( a_{i}=k | x_{i},n,N \right)}$ and $\Phi_{\mathrm{r}}(\gamma)=\sum_{k=\gamma}^{a_{i,\mathrm{max}}}{\mathrm{Pr}\left( a_{i}=k | x_{i},n,N \right)}$ as the left and right tails of the hypergeometric distribution, respectively. To get a \emph{two-tailed} p-value, one can simply double the one-tailed p-value.

Since $a_{i}$ can only take $a_{i,\mathrm{max}} - a_{i,\mathrm{min}} +1$ different values, the corresponding p-values $p_{i}(a_{i})$ are also finitely many. Hence, there exists a minimum attainable p-value defined as $\Psi(x_{i},n,N) = \min\set{p_{i}(\gamma) | a_{i,\mathrm{min}} \leq \gamma \leq a_{i,\mathrm{max}}}$. Since $n$ and $N$ depend only on the labels and are therefore fixed for all patterns, we abbreviate $\Psi(x_{i},n,N)$ as $\Psi(x_{i})$ in the rest of the paper. Given a tentative corrected significance threshold $\delta$ and just based on the margins $x$, $n$ and $N$ of the 2x2 contigency table, one can know that all patterns for which $\Psi(x_{i}) > \delta$ have no chance of being significant and can be pruned from the search space. We will refer to those patterns as \emph{untestable}, while those satisfying $\Psi(x_{i}) \le \delta$ will be said to be \emph{testable}. Even more importantly, because those patterns can never be significant, they do not need to be included in the Bonferroni correction factor. Precisely, let $\mathcal{I}_{T}(\delta)$ be the set of patterns testable at level $\delta$, that is, $\mathcal{I}_{T}(\delta) = \left\{i \in \left\{1,\hdots,D\right\} | \Psi(x_{i}) \le \delta \right\}$ and $m(\delta)=\left\vert \mathcal{I}_{T}(\delta) \right\vert$. Then, following the same steps used to derive the Bonferroni correction, one can prove that $\mathrm{FWER} \le \delta m(\delta)$. Thus, an improved corrected significance threshold can be found as $\delta^{*} = \max\set{\delta | m(\delta) \le \alpha}$. Since $m(\delta) \ll D$ in most real-world datasets, this improvement can bring a drastic increase in statistical power.

One fundamental observation, not emphasised neither in \cite{Tarone} nor \cite{TeradaPNAS}, is that it is essential that the model under the null hypothesis for Fisher's exact test is a probability distribution conditioned on the table marginals. Otherwise, the whole method would not be mathematically sound. Since $\Psi(x_{i})$ conveys information about $x_{i}$, $n$ and $N$, if the distribution of the test statistic under the null hypothesis was not conditional on the margins, knowledge about $\Psi(x_{i})$ could potentially distort the distribution of null p-values due to ``information leaking''. Intuitively, one relies on using test statistics for which evaluating the minimum attainable p-value does not involve any magnitudes modelled as random variables under the null hypothesis or, if it does, those must be provably statistically independent of the test statistic from which the p-values are computed.

{\bf M: The following subsection can be skipped}
\subsection*{Application of Tarone's correction to data mining}

Despite being an elegant way to attenuate the loss of statistical power in setups with discrete test statistics, the method as presented in \cite{Tarone} proposes to solve the optimisation problem leading to $\delta^{*}$ by computing $\Psi(x_{i})$ for each pattern in order to evaluate $m(\delta)$ as many times as needed in a linear search. Needless to say, in a data mining context, such approach is unfeasible except for toy examples, as it would require mining and computing the support of every single pattern in the dataset. The computational unfeasibility of the original method resulted in it being largely ignored by the data mining community until very recently. In \cite{TeradaPNAS}, the authors propose an ingenious way to transform the original optimisation problem into a sequence of frequent pattern mining problems. First of all, they claim the necessity of using a surrogate lower bound $\hat{\Psi}(x_{i})$ for the minimum attainable p-value function such that $\hat{\Psi}(x_{i}) \le \Psi(x_{i})$ holds and ensuring that  $\hat{\Psi}(x_{i})$ is monotonically decreasing in $[0,N]$. They define $\hat{\Psi}(x_{i})$ in such a way\footnote{$\hat{\Psi}(x_{i}) = \begin{cases}\Psi(x_{i}) & 0 \leq x_{i} \leq n \\1 \Big/ \binom{N}{n} & n < x_{i} \leq N \\\end{cases}$} that all patterns for which $x_{i}>n$ are considered testable even if that is not necessarily the case. In other words, one would fetch a set of ``potentially testable'' patterns $\hat{\mathcal{I}}_{T}(\delta) = \left\{i \in \left\{1,\hdots,D\right\} | \hat{\Psi}(x_{i}) \le \delta \right\}$ satisfying\footnote{In \cite{TeradaPNAS}, the authors claim that occurrences of untestable patterns in $\mathcal{I}_{T}(\delta)$ are rare enough to be a major concern, which is indeed true for many problems of interest. Nevertheless, it is also possible to construct cases in which the opposite situation occurs. For instance, if itemsets or substrings were to be combined via union rather than intersection when generating new patterns to be tested.} $\mathcal{I}_{T}(\delta) \subset \hat{\mathcal{I}}_{T}(\delta)$. Nonetheless, as a result of decreasing monotonicity of $\hat{\Psi}$, we can introduce $\sigma(\delta)=\inf \left\{x_i | \hat{\Psi}(x_{i}) \le \delta \right\}$ which enables us to rewrite $\hat{\mathcal{I}}_{T}(\delta)$ as $\hat{\mathcal{I}}_{T}(\sigma(\delta)) = \left\{i \in \left\{1,\hdots,D\right\} | x_{i} \ge \sigma(\delta) \right\}$. Defining $\hat{m} (\sigma)=|\hat{\mathcal{I}}_{T}(\sigma(\delta)) |$, the optimisation problem can then be rewritten as $\sigma^{*} = \min\left\{\sigma | \hat{\Psi}(\sigma) \hat{m}(\sigma) \le \alpha\right\}$.  The number of testable hypothesis is given by $\hat{m}(\sigma^{*})$ and the corrected significant threshold can be recovered as $\hat\delta^{*}=\frac{\alpha}{\hat{m}(\sigma^{*})}$ In \cite{TeradaPNAS}, the authors tackle this reformulation of the original problem with a decremental search strategy, letting $\sigma=N$ at initialisation and solving a sequence of frequent pattern mining problems, using the miner as a black box in order to evaluate $\hat{m}(\sigma)$ for each $\sigma$ until the condition $\hat{\Psi}(\sigma) \hat{m}(\sigma) \le \alpha$ is violated for some value of $\sigma$. When that occurs, one can conclude that $\sigma^{*} = \sigma+1$.

This new strategy has lead to the first successful instance of statistically sound data mining, by being able to successfully obtain p-values quantifying the strength of association between patterns and labels for many small and mid-sized real-world datasets. In order to tackle larger problems, \textbf{F: Cite Mahito's paper} and \cite{Minato} simultaneously proposed changing the search strategy to an incremental scheme with some form of early stopping; the first in the context of subgraph mining and the latter to deal with itemset mining problems. The basic concept is to initialise $\sigma=1$ and iteratively increase $\sigma$ every time the condition $\hat{\Psi}(\sigma) \hat{m}(\sigma) \le \alpha$ is found to be violated. The frequent pattern mining algorithm does not need to be restarted every time $\sigma$ changes, making the whole process efficient. Empirically, this new strategy has been shown to bring a large runtime reduction in both scenarios. Whether the computational complexity can be further reduced beyond this novel strategy in order to deal with even larger and denser datasets remains an interesting open problem.

\subsection*{Addressing dependence between test statistics}

However, there are other pressing challenges for statistically sound data mining beyond runtime considerations. One particularly important open question, completely unaddressed by LAMP regardless of the search strategy used, is how to model the correlation structure between test statistics. In data mining settings such as the ones described in this work, it is intuitively clear that a large amount of patterns will in fact be part of greater patterns and, hence, complex correlation structures involving the different $D$ test statistics will exist. 

One way to model the problem is by realising that, ideally, one would wish to solve $\delta^{*} = \max\set{\delta | \mathrm{FWER}(\delta) \le \alpha}$. Since evaluating $\mathrm{FWER}(\delta)$ is a complex task, all methods exposed so far use a certain quantity as a surrogate upper bound of the FWER instead. For instance, Bonferroni's correction corresponds to using $f(\delta) = \delta D$, whereas the method described in \cite{Tarone} employs $f(\delta) = \delta m(\delta)$. Nevertheless, those upper bounds are often too conservative, resulting in a significant loss of statistical power. It is therefore of great interest to develop algorithms to solve the original problem, without using any upper bound on the FWER as a surrogate. 

It is straightforward to show that the FWER can also be expressed as $\mathrm{FWER}(\delta) = \mathrm{CDF}_{\Omega}(\delta)$ where $\Omega$ is the Random Variable $\Omega = \min\set{p_{i} | i \in \mathcal{K}} | H_{0}^{\mathcal{K}}$, $H_{0}^{\mathcal{K}} = \cap_{i \in \mathcal{K}}{H_{0}^{(i)}}$ and $\mathcal{K}$ is the set of true null hypotheses. Moreover, under a certain technical condition known as the subset pivotality condition, the FWER can also be obtained as the CDF of the random variable $\Omega^{\prime} = \min\set{p_{i} | i \in \set{1,\hdots,D}} | \mathbf{H}_{0}$, with $\mathbf{H}_{0} = \cap_{\set{1,\hdots,D}}{H_{0}^{(i)}}$, which is simpler as it does not depend on the (unknown) ground truth state. Since most often there is no analytic formula available for the distribution of $\Omega^{\prime}$, , nor its CDF, one resorts to resampling methods to approximate it. In the context of statistical association testing, a permutation based resampling scheme proposed by Westfall and Young \cite{WYBook} is one of the most popular approaches. The idea is as follows: if one has to test the association of D random variables $\left\{S_{i}\right\}_{i=1}^{D}$ with another random variable $Y$, a simple way of generating samples of the p-values under the global null (i.e. to generate samples of $\Omega^{\prime}$) is by randomly shuffling (permuting) the observations of $Y$ with respect to those of the random variables $\left\{S_{i}\right\}_{i=1}^{D}$. The permuted datasets obtained that way are effectively samples of the distribution $\mathrm{Pr}\left(\left\{S_{i}\right\}_{i=1}^{D}\right)\mathrm{Pr}(Y)$ and, therefore, correspond to samples obtained from the global null hypothesis that all variables $\left\{S_{i}\right\}_{i=1}^{D}$ are independent of $Y$. Those can then be used to obtain samples from $\mathrm{PDF}(\Omega^{\prime})$ by computing the respective p-values and taking the minimum across all patterns in the database, i.e. $p_{\mathrm{min}}= \min\set{\tilde{p}_{i} | i \in \set{1,\hdots,D}} \sim \mathrm{PDF}(\Omega^{\prime})$, where $\tilde{p}_{i}$ is the p-value resulting from evaluating the association between $S_{i}$ and one realisation of the permuted class labels $\widetilde{Y}$.

While conceptually simple, the Westfall-Young permutation scheme can be extremely computationally demanding. Generating a single sample from $\mathrm{PDF}(\Omega^{\prime})$ naively requires computing the p-values corresponding to all $D$ patterns using a specific permuted version of the class labels, $\widetilde{Y}$. Besides, to get a reasonably good empirical approximation to $\mathrm{FWER}(\delta) = \mathrm{CDF}_{\Omega^{\prime}}(\delta)$, one needs several samples $p_{\mathrm{min}}  \sim \mathrm{PDF}(\Omega^{\prime})$. As it will be shown in the experimental section, a number of samples in the order of $J=10^{3}$ or $J=10^{4}$ is needed to get reliable results. 

If the test statistics are discrete and the minimum attainable p-values can be computed, then one can reuse the ideas behind LAMP to reduce the computational burden which the Westfall-Young permutation-based procedure entails.

Terada et. al. were the first to propose such an algorithm, called FastWY \cite{TeradaIEEE}. It is based on the following observation: if the p-values for all patterns in $\hat{\mathcal{I}}_{T}(\sigma)$ are known and $p_{\mathrm{min}}=\min\set{\tilde{p}_{i} | i \in \hat{\mathcal{I}}_{T}(\sigma)} \le \hat{\Psi}(\sigma)$ then no pattern in $\set{1,\hdots,D} \setminus \hat{\mathcal{I}}_{T}(\sigma)$ can possibly attain a p-value smaller than $p_{\mathrm{min}}$ and the search can be stopped early. That property is exploited to sample from $\mathrm{PDF}(\Omega^{\prime})$ without having to explicitly compute all $D$ p-values. FastWY is based on a decremental search scheme starting with $\sigma=n$. First, a frequent pattern miner is used as a black box to retrieve the set $\hat{\mathcal{I}}_{T}(\sigma)$. Then, the p-values $\tilde{p}_{i}$ are computed $\forall i \in \hat{\mathcal{I}}_{T}(\sigma)$ and $p_{\mathrm{min}}=\min\set{\tilde{p}_{i} | i \in \hat{\mathcal{I}}_{T}(\sigma)}$ is evaluated. If $p_{\mathrm{min}} \le \hat{\Psi}(\sigma)$, no other pattern would be able to make $p_{\mathrm{min}}$ smaller and, therefore, $p_{\mathrm{min}}$ constitutes an exact sample from $\mathrm{PDF}(\Omega^{\prime})$. On the contrary, if $p_{\mathrm{min}} > \hat{\Psi}(\sigma)$, $\sigma$ is decreased by one unit and the whole procedure is repeated until the condition $p_{\mathrm{min}} \le \hat{\Psi}(\sigma)$ is satisfied.

If $J$ permutations are needed to empirically estimate the FWER, the procedure has be to repeated $J$ times. That includes the whole sequence of frequent mining problems needed to retrieve the sets $\hat{\mathcal{I}}_{T}(\sigma)$ for all values of $\sigma$ used throughout the decremental search. Given the usual range of values for $J$, such an approach is just as unfeasible in practice as the original brute force baseline.

Interestingly, careful inspection of the code kindly shared by the authors in their website reveals that the actual implementation of the algorithm is different from the description in \cite{TeradaIEEE}. Indeed, to alleviate the inadmissible burden of repeating the whole frequent pattern mining process $J$ times, the authors resort to storing each of the sets $\hat{\mathcal{I}}_{T}(\sigma)$ in memory, along\footnote{In fact, storing $S_{i} \; \forall i \in \hat{\mathcal{I}}_{T}(\sigma)$ is the main problem almost exclusively, as the patterns themselves do not really need to be stored in memory.} with the corresponding realisations of the variables $S_{i} \; \forall i \in \hat{\mathcal{I}}_{T}(\sigma)$. Clearly, this decision corresponds to a drastic trade-off between runtime and memory usage since, as we will show empirically, there exist many databases for which the amount of information to be stored when following that approach is too large to fit even in large servers equipped with 512GB of RAM. Furthermore, we will also demonstrate that the algorithm resulting from trading off memory in exchange for runtime is still slow even for mid-sized datasets and can be greatly improved.
% * <llinares.felipe@gmail.com> 2014-12-20T00:16:35.979Z:
%
%  Do you think that the previous paragraph (And the beginning of the next section) are too harsh? I want to point out the limitations of Terada's work enough for us to have a good chance of acceptance, but I don't want to bash her work. I'd say right now it sounds a bit too critical...
%
When referring to the FastWY algorithm in \cite{TeradaIEEE} throughout the remaining of this paper, we mean the runtime-optimised version of the algorithm, given that the algorithm exactly as described in \cite{TeradaIEEE} simply cannot be run in a reasonable amount of time.

==> relatedwork2.tex <==
\section{Related work}
\label{sec:relatedwork}

In pattern mining, every p-value can be obtained from a $2 \times 2$ contingency table:
\begin{center}
	\begin{tabular}{|c|c|c|c|}
		\hline
		Variables & $S_{i}=1$ & $S_{i}=0$ & Row totals\\
		\hline
		$Y=1$ & $a_{i}$ & $n-a_{i}$ & $n$ \\
		\hline
		$Y=0$ & $x_{i}-a_{i}$ & $N+a_{i}-n-x_i$ & $N-n$ \\
		\hline
		Col totals & $x_{i}$ & $N-x_{i}$ & $N$ \\
		\hline
	\end{tabular}
\end{center}
$2 \times 2$ contingency tables are generally used to evaluate the strength of the association between two binary variables. In our case, those correspond to the class labels $Y$ and a variable $S_{i}$ that indicates whether the $i$-th pattern is present or not for each of the $N$ objects in the database ($S_i = 1$ meaning that the $i$-th pattern exists in the object). In a given database, $N$ denotes the total number of objects, $n$ the number of objects with class label $Y = 1$, $x_{i}$ the number of objects containing the $i$-th pattern, and $a_{i}$ the number of objects with class label $Y = 1$ containing the $i$-th pattern. Without loss of generality, we assume that the class labels are encoded so that $n \le N-n$.  

Let us use {\em Fisher's exact test}~\cite{FisherExactTest} to derive the test statistic, as it is one of the most popular methods to obtain a p-value out of a $2 \times 2$ contingency table. Fisher's exact test assumes that all marginals $x_{i}$, $n$, and $N$ are fixed. Thus, the table has only one degree of freedom left and one can model it as a one-dimensional count $a_{i}$. Under those assumptions, it can be shown that the underlying data-generating model under the null hypothesis of statistical independence between $S_{i}$ and $Y$ is a hypergeometric random variable. 

Mathematically, $\mathrm{Pr}\left(a_{i}=k | x_{i},n,N\right) = \binom{n}{k}\binom{N-n}{x_{i}-k} / \binom{N}{x_{i}}$ with support on $a_{i,\mathrm{min}} \leq k \leq a_{i,\mathrm{max}}$, $a_{i,\mathrm{min}}=\max\{0,x_{i}+n-N\}$ and $a_{i,\mathrm{max}}=\min\{n,x_{i}\}$. If for a given pattern we observe $a_{i}=\gamma$, the corresponding \emph{one-tailed} p-value can be obtained as $p_{i}(\gamma) = \min \{\Phi_{\mathrm{l}}(\gamma),\Phi_{\mathrm{r}}(\gamma)\}$, where we define $\Phi_{\mathrm{l}}(\gamma)=\sum_{k=a_{i,\mathrm{min}}}^{\gamma}{\mathrm{Pr}\left( a_{i}=k | x_{i},n,N \right)}$ and $\Phi_{\mathrm{r}}(\gamma)=\sum_{k=\gamma}^{a_{i,\mathrm{max}}}{\mathrm{Pr}\left( a_{i}=k | x_{i},n,N \right)}$ as the left and right tails of the hypergeometric distribution, respectively. To get a \emph{two-tailed} p-value, one can simply double the one-tailed p-value.

Since $a_{i}$ can only take $a_{i,\mathrm{max}} - a_{i,\mathrm{min}} +1$ different values, the corresponding p-values $p_{i}(a_{i})$ are also finitely many. Hence, there exists a {\em minimum attainable p-value} defined as $\Psi(x_{i},n,N) = \min\set{p_{i}(\gamma) | a_{i,\mathrm{min}} \leq \gamma \leq a_{i,\mathrm{max}}}$. As $n$ and $N$ depend only on the labels and are therefore fixed for all patterns, we abbreviate $\Psi(x_{i},n,N)$ as $\Psi(x_{i})$ in the rest of the paper. 

Tarone \cite{Tarone} was the first to propose exploiting that property in order to reduce the loss of statistical power due to multiple testing. Given a tentative corrected significance threshold $\delta$, and just based on the margins $x$, $n$ and $N$ of the 2x2 contingency table, one can know that all patterns for which $\Psi(x_{i}) > \delta$ have no chance of being significant and can be pruned from the search space. Even more importantly, because those patterns can never be significant, they do not need to be included in the Bonferroni correction factor. Precisely, let $\mathcal{I}_{T}(\delta) = \left\{i \in \left\{1,\hdots,D\right\} | \Psi(x_{i}) \le \delta \right\}$ and $m(\delta)=\left\vert \mathcal{I}_{T}(\delta) \right\vert$. Then, following the same steps used to derive the Bonferroni correction, one can prove that $\mathrm{FWER} \le \delta m(\delta)$. Thus, an improved corrected significance threshold can be found as $\delta^{*} = \max\set{\delta | \delta m(\delta) \le \alpha}$. Since $m(\delta) \ll D$ in most real-world datasets, this improvement can bring a drastic increase in statistical power.

This improved Bonferroni correction for discrete data, as proposed in \cite{Tarone}, would require computing $\Psi(x_{i})$ for each pattern in order to evaluate $m(\delta)$ as many times as needed in a linear search. Needless to say, in a data mining context, that approach is unfeasible as it would require mining and computing the support of every single pattern in the dataset. The computational unfeasibility of the original method resulted in it being largely ignored by the data mining community until the 2013 breakthrough paper by Terada et al.~\cite{TeradaPNAS}. There, the authors propose the Limitless-Arity Multiple-testing Procedure (LAMP), a branch-and-bound algorithm which, under some simplifications, is able to apply the method described in~\cite{Tarone} to data mining problems of the form considered in this paper.

Nevertheless, neither the method described in \cite{Tarone} nor its efficient implementation in \cite{TeradaPNAS} address the dependence between test statistics. Consequently, they are strictly suboptimal testing procedures which lose statistical power by overestimating the FWER.

To the best of our knowledge, Terada et al.~\cite{TeradaIEEE} have been the only ones so far to propose a permutation-based testing scheme for significant pattern mining. There the authors propose FastWY, an algorithm which again uses the concept of minimum attainable p-value. Just like LAMP, FastWY requires the function $\Psi(x_{i})$ to be monotonically decreasing in $[0,N]$. As that is not the case, both LAMP and FastWY use a surrogate lower bound $\hat{\Psi}(x_{i})$ defined as
\begin{flalign*}
\hat{\Psi}(x_{i}) = \begin{cases}\Psi(x_{i}) & 0 \leq x_{i} \leq n, \\1 \big/ \binom{N}{n} & n < x_{i} \leq N \\\end{cases}
\end{flalign*}
and define $\hat{\mathcal{I}}_{T}(\delta) = \{\,i \in \left\{1,\hdots,D\right\} \mid \hat{\Psi}(x_{i}) \le \delta\,\}$, which always satisfies $\mathcal{I}_{T}(\delta) \subset \hat{\mathcal{I}}_{T}(\delta)$. In other words, the set of patterns they retrieve might contain some unnecessary patterns.
% so that all patterns with $x_{i}>n$ are considered to be testable even if that is not necessarily the case. In other words, with their approach one would fetch a set of ``potentially testable'' patterns $\hat{\mathcal{I}}_{T}(\delta) = \{\,i \in \left\{1,\hdots,D\right\} \mid \hat{\Psi}(x_{i}) \le \delta\,\}$ satisfying $\mathcal{I}_{T}(\delta) \subset \hat{\mathcal{I}}_{T}(\delta)$. 
Nonetheless, as a result of the monotonicity of $\hat{\Psi}$, we can rewrite $\hat{\mathcal{I}}_{T}(\delta)$ as $\hat{\mathcal{I}}_{T}(\sigma(\delta)) = \{\,i \in \left\{1,\hdots,D\right\} \mid x_{i} \ge \sigma(\delta)\,\}$ using $\sigma(\delta)=\inf \{\,x_i \mid \hat{\Psi}(x_{i}) \le \delta\,\}$. This new formulation is important because $\hat{\mathcal{I}}_{T}(\sigma(\delta))$ can be readily seen to correspond to an instance of \emph{frequent pattern mining with support $\sigma(\delta)$}, a well studied problem in data mining.

That property is the basis of LAMP and is also relevant for FastWY as follows: If the p-values for all patterns in $\hat{\mathcal{I}}_{T}(\sigma)$ are known and $p_{\mathrm{min}}=\min\set{\tilde{p}_{i} | i \in \hat{\mathcal{I}}_{T}(\sigma)} \le \hat{\Psi}(\sigma)$, no pattern in $\set{1,\hdots,D} \setminus \hat{\mathcal{I}}_{T}(\sigma)$ can possibly attain a p-value smaller than $p_{\mathrm{min}}$ and the search can be stopped early.

That can be exploited to sample from $\mathrm{PDF}(\Omega^{\prime})$ without having to explicitly compute all $D$ p-values. It is based on a decremental search scheme starting with $\sigma=n$. First, a frequent pattern miner is used as a black box to retrieve the set $\hat{\mathcal{I}}_{T}(\sigma)$. Then, the p-values $\tilde{p}_{i}$ are computed for all $i \in \hat{\mathcal{I}}_{T}(\sigma)$ and $p_{\mathrm{min}}=\min\set{\tilde{p}_{i} | i \in \hat{\mathcal{I}}_{T}(\sigma)}$ is evaluated. If $p_{\mathrm{min}} \le \hat{\Psi}(\sigma)$, no other pattern would be able to make $p_{\mathrm{min}}$ smaller and, therefore, $p_{\mathrm{min}}$ constitutes an exact sample from $\mathrm{PDF}(\Omega^{\prime})$. On the contrary, if $p_{\mathrm{min}} > \hat{\Psi}(\sigma)$, $\sigma$ is decreased by one unit and the whole procedure is repeated until the condition $p_{\mathrm{min}} \le \hat{\Psi}(\sigma)$ is satisfied.

If $J$ permutations are needed to empirically estimate the FWER, the procedure has be to repeated $J$ times. That includes the whole sequence of frequent mining problems needed to retrieve the sets $\hat{\mathcal{I}}_{T}(\sigma)$ for each value of $\sigma$ used throughout the decremental search. Given the usual range of values for $J$, such an approach is just as unfeasible in practice as the original brute force baseline.

Interestingly, careful inspection of the code kindly shared by the authors in their website reveals that the actual implementation of the algorithm is different from the description in \cite{TeradaIEEE}. Indeed, to alleviate the inadmissible burden of repeating the whole frequent pattern mining process $J$ times, the authors resort to storing the realisations of the variables $S_{i}$ for all $i \in \hat{\mathcal{I}}_{T}(\sigma)$ and every value of $\sigma$ explored during the decremental search. Clearly, this decision corresponds to a drastic trade-off between runtime and memory usage since, as we will show empirically, there exist many databases for which the amount of information to be stored when following that approach is too large to fit even in large servers equipped with 512GB of RAM. Furthermore, we will also demonstrate that the algorithm resulting from trading off memory in exchange for runtime is still slow even for mid-sized datasets and can be greatly improved.

When referring to the FastWY algorithm in \cite{TeradaIEEE} throughout the remaining of this paper, we mean the runtime optimized version of the algorithm, given that the algorithm exactly as described in \cite{TeradaIEEE} simply cannot be run in a reasonable amount of time.


